Integrating Multimodal Information in Large Pretrained Transformers

Recent Transformer-based contextual word representations, including BERT and XLNet, have shown state-of-the-art performance in multiple disciplines within NLP. Fine-tuning the trained contextual models on task-specific datasets has been the key to achieving superior performance downstream. While fine-tuning these pre-trained models is straightforward for lexical applications (applications with only language modality), it is not trivial for multimodal language (a growing area in NLP focused on modeling face-to-face communication). Pre-trained models don't have the necessary components to accept two extra modalities of vision and acoustic. In this paper, we proposed an attachment to BERT and XLNet called Multimodal Adaptation Gate (MAG). MAG allows BERT and XLNet to accept multimodal nonverbal data during fine-tuning. It does so by generating a shift to internal representation of BERT and XLNet; a shift that is conditioned on the visual and acoustic modalities. In our experiments, we study the commonly used CMU-MOSI and CMU-MOSEI datasets for multimodal sentiment analysis. Fine-tuning MAG-BERT and MAG-XLNet significantly boosts the sentiment analysis performance over previous baselines as well as language-only fine-tuning of BERT and XLNet. On the CMU-MOSI dataset, MAG-XLNet achieves human-level multimodal sentiment analysis performance for the first time in the NLP community.

==> sections/cache.tex <==
since fine-tuning these Multimodal language analysis is an emerging research area in NLP which strives to model face-to-face communication from modalities of language, vision and acoustic. Fine-tuning BERT and XLNet is not 


This research area models the face-to-face communication as a signal consisting of language, visual and acoustic modalities. With the advent of transformer-based models such as , language modality  provide strong contextual language representations after training on large-scale unlabeled corpora. Fine-tuning both models has shown promising results in building state-of-the-art models for diverse NLP tasks like question answering and language inference. However, fine-tuning them in the presence of information from other modalities remains an open research problem. In this paper, we inject multimodal information within the input space of both models for modeling multimodal language. The proposed injection method allows BERT to reach a new state of the art of $84.38\%$ binary accuracy on CMU-MOSI dataset (multimodal sentiment analysis) with a gap of 5.98 percent to the previous state of the art and 1.02 percent to the text-only BERT. \commentWA{Needs to give a unified results for XLnet on both mosi and mosei,plus also needs to take care of new metric.}



Transformer-XL~\cite{dai2019transformer} address two problems of Vanilla Transformer: failure to capture long term dependency and context fragmentation -- inability to predict first few symbols well.
It does so with a recurrence mechanism designed to pass context information from one segment to the next, thus capturing long term dependency. It also uses a relative positional encoding mechanism to enable state reuse without causing temporal confusion.



\noindent \textbf{Multimodal Variation of Language Representations}: Words can have different meaning when they appears with different non-verbal intents \cite{zadeh2017tensor,wang2018words}. Dynamic shifting of word representations based on their accompanying non-verbal context has shown promising performance on the task of multimodal sentiment and emotion recognition \cite{wang2018words}.  

\subsection{Multimodal XLNet}
\label{model:multi_xlnet}
We will discuss our proposed \textbf{M-XLNet} model in two steps: a short introduction to the XLNet model followed by our approach of injecting audio-visual information in the XLNet network.

\subsection{Multimodal BERT}
\label{model:multi-bert}
We discuss our proposed M-BERT model in two steps: a short overview on the BERT model and our approach on injecting audio-visual information in the BERT network.

\textbf{M-BERT:} In this variant, we inject audio-visual information with text in BERT structure through the \textbf{Multimodal Shifting Gate} (Sec~\ref{model:m-bert}).


We can also determine the effect of non-verbal information injection in BERT structure by comparing the performance of M-BERT with BERT.




We use the following variants of BERT to study multimodal sentiment analysis task:

\textbf{BERT:} In this variant, we fine-tune the standard BERT network described in \ref{model-bert} using text information only. 


\noindent \textbf{Fine-tuning Transformer Models}
VideoBERT~\cite{sun2019videobert} jointly models a video and the corresponding text in a self-supervised manner and achieves state-of-the-art performance in a wide variety of tasks ranging from action classification to video captioning. To model the textual data, it uses a per-trained BERT model and successfully fine-tunes that to capture context from video data as well.\commentK{This paper is not published yet. will this paper undermine the novelty of our work?} However,~\cite{tan2019lxmert} achieved better performance by training their model from scratch instead of fine-tuning in the video-and-language reasoning tasks. 


% which provides better contextual modeling only.

% Furthermore, it allow us to understand the performance of BERT contextual representation for multimodal language modeling.

% Using these two variants, we can determine how non-verbal information infusion through the \textbf{Multimodal Shifting Gate} can improve performance on better contextual language modeling of BERT.

% These two variants allow us to separate the effects of two sources of performance gain: better contextual language modeling of BERT and non-verbal information infusion through the \textbf{Multimodal Shifting Gate} strategy. Both of them fine-tune the pre-trained BERT model with extensive hyper-parameter search.

Learning Rate: [1e-5,1.5e-5,2e-5,2.5e-5,......6e-5]\\
Gradient Accumulation Steps: [1,2,3,4]\\
Hidden Dropout Prob: [0.1,0.2,0.25,0.3,0.35,0.4,0.45....0.6]\\
Beta Shift: [0.25, 0.3, 0.35, 0.4, 0.45, 0.5, 0.6, 0.7, 0.8, 0.9, 1, 1.5, 1.8, 2, 2.2, 2.5, 2.8, 3, 3.2, 3.4, 3.6, 3.8, 4, 4.5, 4.8, 5, 5.5, 5.8, 6, 6.2, 6.4, 7, 8, 10, 12, 14, 16, 20, 22, 24, 28, 30, 32, 40, 44, 50, 60, 70, 80, 100]\\

==> sections/todo.tex <==
SANGWU:
    XLNET for MOSI MOSEI, BERT for MOSEI to Amir
    XLNET further experiments on MOSI to beat human performance.
    Continue experiments on MOSEI
    
Amir: 
    Get Emotions from Hubert
    
Kamrul and Wasifur:
    Make changes to the write up
    bert-encoder figure is underwhelming. There needs to be a stack of encoders, 

==> subsections/bert.tex <==
\subsection{BERT}
\label{model-bert}
 We use the variant of BERT used for \textit{Single Sentence Classification Tasks}~\cite{devlin2018bert}. First, \textit{input embeddings} are generated from a sequence of word-piece tokens by adding token embeddings, segment embeddings and position embeddings (we define this component as \textbf{BERT Input Embedder}). Then \textbf{BERT Encoder} applies multiple self-attention layers on top of these input embeddings to attend to inputs with respect to each other. A special [CLS] token is appended in front of the input token sequence. So, for a $N$ length input sequence, we get $N$+1 vectors from the \textbf{BERT Encoder} -- the first of them representing the class of this input sequence. This class vector is used to predict the label of the input.
% The BERT model includes two major components: \textbf{BERT Input Embedder} and \textbf{BERT Encoder}\cite{devlin2018bert}\textcolor{red}{NEED FURTHER DISCUSSION}. \textbf{BERT Input Embedder} takes a sequence of word-piece tokens and generate \textbf{Input Embeddings} as a sum of token embeddings, segment embeddings and position embeddings. \textbf{BERT Encoder} applies multiple self-attention layers on top of these \textbf{Input Embeddings} to attend to inputs with respect to each other. We use the variant of BERT used for \textit{Single Sentence Classification Tasks}. In this variant, special [CLS] token is appended in front of the input token sequence. So, for a $N$ length input sequence, we get $N$+1 vectors from the \textbf{\textit{BERT Encoder}} -- the first of them representing the class of this input sequence. We use that vector to predict the class label of the input.  

==> subsections/m_xlnet.tex <==






==> subsections/vanilla_transformer.tex <==



==> subsections/xlnet.tex <==
\subsection{XLNet}
\label{model:xlnet}
XLNet will be here

==> tables/res_mosei.tex <==
\begin{table}[t!]
\begin{center}
\small
\fontsize{9}{10}\selectfont
\setlength{\tabcolsep}{5.5pt}
\renewcommand{\arraystretch}{1.2}
\begin{tabular}{l|cc|cc}
%\Xhline{3\arrayrulewidth}
Task Metric & BA$\uparrow$ & F1$\uparrow$ & MAE$\downarrow$ & Corr$\uparrow$ \\
\hline
\multicolumn{5}{|c|}{Original (glove)} \\
\hline 
TFN & 74.8/-- & 75.4/--  & 0.72/-- & 0.52/-- \\
MARN & 75.9/-- & 75.8/--  & 0.73/-- & 0.51/-- \\
MFN & 76.0/-- & 76.0/--  & 0.72/-- & 0.52/-- \\
RMFN & 77.1/-- & 77.0/--  & 0.968/-- & 0.625/-- \\
MulT & --/82.5 & --/82.3 & 0.580 & 0.703\\
\hline 
\hline
\multicolumn{5}{|c|}{BERT} \\
\hline 
TFN & X/X & X/X  & X & X \\
MARN & X/X & X/X  & X & X \\
MFN & 78.2/80.1 & 78.9/80.5  & 0.597/— & 0.702/— \\
RMFN & --/-- & --/--  & --/-- & --/-- \\
LFN & X/X & X/SC  & X & X \\
MulT(Hubert) & 82.5 & 82.3 & 0.580 & 0.703\\
\hline 
BERT& 83.9/86.1 & 83.9/86.0  & 0.537 & 0.764\\
M-BERT & \textbf{84.7}/86.0 & \textbf{84.5}/86.0 & \textbf{0.539} & \textbf{0.766} \\
\hline 
\hline
$\Delta_{SOTA}$ & $\uparrow$ \textbf{X}  & $\uparrow$ \textbf{X}  & $\downarrow$ \textbf{X} & $\uparrow$\textbf{X}\\ 
\hline
\multicolumn{5}{|c|}{XLNet} \\
\hline 
TFN & X/X & X/X  & X & X \\
MARN & X/X & X/X  & X & X \\
MFN & X/X & X/X  & X & X \\
RMFN & --/-- & --/--  & --/-- & --/-- \\
LFN & X/X & X/X  & X & X \\
MulT &  X/X & X/X & X & X \\
\hline 
XLNet& 85.4/86.4 & 85.2/86.4 & 0.534 & 0.770\\
M-XLNet & \textbf{85.6}/86.8 & \textbf{85.7}/86.8 & \textbf{0.538} & \textbf{0.774} \\
\hline
Human & X/- & X/- & X & X \\
\hline
\hline
$\Delta_{Human}$ & $\uparrow$ \textbf{X}  & $\uparrow$ \textbf{X}  & $\downarrow$ \textbf{X} & $\uparrow$\textbf{X}\\ 
$\Delta_{BERT}$ & $\uparrow$ \textbf{X}  & $\uparrow$ \textbf{X}  & $\downarrow$ \textbf{X} & $\uparrow$\textbf{X}\\ 
$\Delta_{SOTA}$ & $\uparrow$ \textbf{X}  & $\uparrow$ \textbf{X}  & $\downarrow$ \textbf{X} & $\uparrow$\textbf{X}\\ 
\hline
\end{tabular}
\end{center}
%SOTA1=RMFN, SOTA2=MFN, SOTA3=MARN 
\caption{ \commentW{ Amir, RMFN does not have mosei}\\\commentW{What is the MulT in BERT and XLNet section?}Sentiment prediction results on CMU-MOSEI. SOTA1, SOTA2 and SOTA3 refer to the previous best, second best and third best state of the art models respectively. Best results are highlighted in bold and $\Delta_{SOTA}$ represents the change in performance of M-BERT model over SOTA1. Our model significantly outperforms the current SOTA across all evaluation metrics.}
\label{table:mosei_performance}


\end{table}
